f-GANs in an Information Geometric Nutshell

Nowozin \textit{et al} showed last year how to extend the GAN \textit{principle} to all $f$-divergences. The approach is elegant but falls short of a full description of the supervised game, and says little about the key player, the generator: for example, what does the generator actually converge to if solving the GAN game means convergence in some space of parameters? How does that provide hints on the generator's design and compare to the flourishing but almost exclusively experimental literature on the subject? In this paper, we unveil a broad class of distributions for which such convergence happens --- namely, deformed exponential families, a wide superset of exponential families --- and show tight connections with the three other key GAN parameters: loss, game and architecture. In particular, we show that current deep architectures are able to factorize a very large number of such densities using an especially compact design, hence displaying the power of deep architectures and their concinnity in the $f$-GAN game. This result holds given a sufficient condition on \textit{activation functions} --- which turns out to be satisfied by popular choices. The key to our results is a variational generalization of an old theorem that relates the KL divergence between regular exponential families and divergences between their natural parameters. We complete this picture with additional results and experimental insights on how these results may be used to ground further improvements of GAN architectures, via (i) a principled design of the activation functions in the generator and (ii) an explicit integration of proper composite losses' link function in the discriminator.

==> arxiv-gan-proof-viggan.tex <==


Without loss of generality we can assume that $\sup \mathbb{I}_{P,Q} <
+\infty$. Otherwise, when $\sup \mathbb{I}_{P,Q} = + \infty$,
requesting $\sup \xi(\mathbb{I}_{P,Q}) = +\infty$ ($\forall \xi \in \partial
f$) implies, because $f$
is convex continuous, that $\lim_{\sup
  \mathbb{I}_{P,Q}}f(z) = +\infty$, and so the constraint $I_f(P\|Q) <
+\infty$ essentially enforces zero measure over all infinite density ratios.

We make use of \cite[Proposition 1.6.1]{npCF}, now with a
subdifferential which is not Riemann integrable in $M \defeq \sup
\mathbb{I}_{P,Q}$. Notice that we can assume without loss of
generality that $M > 1$ since otherwise, since it is convex and
continuous, $f$ would not be defined for $z> 1$ and $I_f(P\|Q)$
would essentially be infinite unless $Q \geq P$ almost everywhere
(\textit{i.e.} $P$ dominates $Q$ only on sets of zero measure).\\

For any constants
$t^* < M, \epsilon$ such that $\xi(t^*) < +\infty$, let
\begin{eqnarray}
g_{t^*,\epsilon}(z) & \defeq & \int_{1}^{z}
(-\xi(t)+\xi(t^*)+\epsilon)\mathrm{d}t\:\:, 
\end{eqnarray}
where $z \in \mathbb{R}_+$ is any real such that the integral in
$g_{t^*,\epsilon}$ is not improper
(therefore, $z< M$). Let
\begin{eqnarray}
\chi_{t^*,\epsilon}(t) & = & \left\{
\begin{array}{rcl}
\frac{1}{-\xi(t) +\xi(t^*)+\epsilon} & \mbox{ if } & t < t^*\:\:,\\
\frac{1}{\epsilon} & \mbox{ if } & t \geq t^*
\end{array}
\right.\:\:,
\end{eqnarray}
which, if $\epsilon > 0$, is non negative and also increasing
since $\xi $ is increasing. Consider any fixed $z^* \in \mathbb{I}_{P,Q}
\cap (1,\infty)$ with $0<\xi(z^*) < \infty$ and let $t^* \defeq \sup
\{z : \xi(z) \leq \xi(z^*)\}$. We have:
\begin{eqnarray}
g_{t^*,\epsilon}(z) & = & \int_{1}^{z}
(-\xi(t)+\xi(t^*)+\epsilon)\mathrm{d}t\nonumber\\
& = & \int_{1}^{z}
\frac{1}{\chi_{t^*,\epsilon}(t)} \mathrm{d}t + 1_{[z \geq t^*]} \cdot \int_{t^*}^{z}
(-\xi(t)+ \xi(t^*))\mathrm{d}t\nonumber\\
& =  & \int_{1}^{z}
\frac{1}{\chi_{t^*,\epsilon}(t)} \mathrm{d}t  -
1_{[z \geq t^*]} \cdot \int_{t^*}^{z}
(\xi(t)- \xi(t^*))\mathrm{d}t\nonumber\\
 & = & \int_{1}^{z}
\frac{1}{\chi_{t^*,\epsilon}(t)} \mathrm{d}t  -
1_{[z\geq t^*]} \cdot D_{f,
  \xi}\left(\left. z\right\| t^*\right) \label{inv3}\:\:.
\end{eqnarray}
The last identity comes from \cite[Proposition 1.6.1]{npCF} and the
fact that $\xi(t)- \xi(t^*)$ belongs to the subdifferential of the
Bregman divergence whose generator is $f$ \cite{frCF}. We obtain:
\begin{eqnarray}
\lefteqn{\expect_{\X\sim
  Q}\left[f
  \left(\frac{P(\X)}{Q(\X)}\right)\right]}\nonumber\\
 & = & \expect_{\X\sim
  Q}\left[f_{\xi(t^*)+\epsilon}
  \left(\frac{P(\X)}{Q(\X)}\right)\right]\label{cons11}\\
 & = & \expect_{\X\sim
  Q}\left[\lim_{\rho \rightarrow \frac{P(\X)}{Q(\X)}} -\int_{1}^{\rho}
(-\xi(t)+\xi(t^*)+\epsilon) \mathrm{d}t\right]\label{cons12}\\
 & = & \expect_{\X\sim
  Q}\left[\lim_{\rho \rightarrow \frac{P(\X)}{Q(\X)}} -g_{t^*,\epsilon}(\rho)\right]\nonumber\\
 & = & \expect_{\X\sim
  Q}\left[\lim_{\rho \rightarrow \frac{P(\X)}{Q(\X)}}
  \left\{-\int_{1}^{\rho}
\frac{1}{\chi_{t^*,\epsilon}(t)} \mathrm{d}t +
1_{\left[\rho\geq t^*\right]} \cdot D_{f,
  \xi}\left(\left. \rho \right\| t^*\right) \right\}\right]\label{cons13}\\
 & = & \expect_{\X\sim
  Q}\left[-\lim_{\rho \rightarrow \frac{P(\X)}{Q(\X)}}
  \int_{1}^{\rho}
\frac{1}{\chi_{t^*,\epsilon}(t)} \mathrm{d}t\right] + \underbrace{\expect_{\X\sim
  Q}\left[\lim_{\rho \rightarrow \frac{P(\X)}{Q(\X)}}
1_{\left[\rho\geq t^*\right]} \cdot D_{f,
  \xi}\left(\left. \rho \right\| t^*\right) \right]}_{\defeq R(t^*)}\label{cons15}\\
 & = & \expect_{\X\sim
  Q}\left[-\log_{\chi_{t^*,\epsilon}}\left(\frac{P(\X)}{
      Q(\X)}\right)\right] + R(t^*)\label{cons16}\\
 & = & KL_{\chi_{t^*,\epsilon}}(Q\|P) + R(t^*)\label{cons17}\:\:.
\end{eqnarray}
Eq. (\ref{cons11}) follows from Eq. (\ref{inv1}).
Eq. (\ref{cons12}) follows from Eq. (\ref{inv2}).
Eq. (\ref{cons13}) follows from Eq. (\ref{inv3}). We can split the
limits in eq. (\ref{cons15}) because each term in the expectation of
$R(t^*)$ is finite. To see it, since $I_f(P\|Q) < \infty$ and $\sup
\xi (\mathbb{I}_{P,Q}) = +\infty$, we can assume that $f(M) <
+\infty$. Since $\xi(t^*) \geq
0$, then
\begin{eqnarray}
\rho \geq t^* & \Rightarrow & D_{f,
  \xi}\left(\left. \rho \right\| t^*\right) \leq f(M) - f(t^*) \:\:,
\end{eqnarray}
which is indeed finite. It then comes 
\begin{eqnarray}
\expect_{\X\sim
  Q}\left[\lim_{\rho \rightarrow \frac{P(\X)}{Q(\X)}}
1_{\left[\rho\geq t^*\right]} \cdot D_{f,
  \xi}\left(\left. \rho \right\| t^*\right) \right] & = & \expect_{\X\sim
  Q}\left[
1_{\left[\frac{P(\X)}{Q(\X)}\geq t^*\right]} \cdot D_{f,
  \xi}\left(\left. \frac{P(\X)}{Q(\X)} \right\| t^*\right)
\right]\nonumber\\
 & \leq & \expect_{\X\sim
  Q}\left[D_{f,
  \xi}(M\|t^*)
\right] \nonumber\\
 & \leq & f(M) - f(t^*)\:\:.
\end{eqnarray}
Since $f$ is continuous, we get the upperbound on $I_f(P\|Q)$ by choosing $t^*<M$ as
close as desired to $M$. We get the lowerbound by remarking that
$R(t^*) \geq 0$ (a Bregman divergence cannot be negative).

\newpage

\begin{theorem}
Letting
$P\defeq P_{\chi, C}$ and $Q \defeq Q_{\chi, C}$ for short, the following holds:
\begin{eqnarray}
\expect_{\X\sim \tilde{Q}}[\log_\chi(Q(\X)) - \log_\chi(P(\X))] & = &
KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|P) - J(Q)\:\:,
\end{eqnarray} 
with $J(Q) \defeq
KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|Q)$ and $\chi_{\tilde{Q}(\ve{x})}(t) \defeq (1/\tilde{Q}(\ve{x}))\cdot \chi
(t \tilde{Q}(\ve{x}))$.
\end{theorem}
The normalization $Z$ for the escort of $Q$ being
finite, it implies the finiteness of $\tilde{Q}$ almost everywhere

We have
\begin{eqnarray*}
\expect_{\tilde{{Q}}}[-(\log_\chi({P})-\log_\chi({Q}))]
& = &
\expect_{\tilde{{Q}}}[-(\log_\chi({P})-\log_\chi(\tilde{{Q}}))]
+ \expect_{\tilde{{Q}}}[-(\log_\chi(\tilde{{Q}})-\log_\chi({Q}))]\:\:.
\end{eqnarray*}
Also, 
\begin{eqnarray}
(\log_\chi({P})-\log_\chi({\tilde{{Q}}})) & = & \int_{{{1}}}^P
\frac{1}{\chi(t)} \cdot \mathrm{d}t - \int_1^{\tilde{{Q}}}
\frac{1}{\chi(t)} \cdot \mathrm{d}t\nonumber\\
& = & \int_{\tilde{{Q}}}^P
\frac{1}{\chi(t)} \cdot \mathrm{d}t\nonumber\\
 & = & \int_{1}^{\frac{P}{\tilde{{Q}}}}
\frac{\tilde{{Q}}}{\chi(t \tilde{{Q}})} \cdot \mathrm{d}t\nonumber\\
 & = & \int_{1}^{\frac{P}{\tilde{{Q}}}}
\frac{1}{\chi_{\tilde{{Q}}}(t)} \cdot \mathrm{d}t\nonumber\\
 & = & \log_{\chi_{\tilde{{Q}}}}\left(\frac{P}{\tilde{{Q}}}\right)\:\:,
\end{eqnarray}
with 
\begin{eqnarray}
\chi_{\tilde{{Q}}(\ve{x})}(t) & \defeq & \frac{1}{\tilde{{Q}} (\ve{x})}\cdot \chi
(t\tilde{{Q}}(\ve{x}))\label{defCHITILDE} 
\end{eqnarray}
satisfying $\mathrm{d} \chi_{\tilde{{Q}} (\ve{x})} /
\mathrm{d} t = \chi'
(t \tilde{{Q}} (\ve{x}))$ and so is increasing, plus $\chi_{\tilde{{Q}}}$ is
positive iff $\chi$ is positive since $\tilde{{Q}}(\ve{x})\geq 0$, so $\chi_{\tilde{{Q}}}(t)$
defines a
$\chi$-logarithm, also differentiable. Hence,
\begin{eqnarray}
\expect_{\tilde{{Q}}}[-(\log_\chi({P})-\log_\chi(\tilde{{Q}}))] & = & KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|P)\:\:,
\end{eqnarray}
and
\begin{eqnarray}
\expect_{\tilde{{Q}}}[-(\log_\chi({Q}) - \log_\chi(\tilde{{Q}}))] & = & KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|Q)\:\:.
\end{eqnarray}
This ends the proof of point (ii).\\

\newpage

\noindent We prove point (i). We first remark that we have $(-\log_{\chi})'' = \chi' / \chi^2 \geq 0$ and so $-\log_{\chi}$ is convex and $KL_{\chi}(P\|Q)$ is an
$f$-divergence with $f$ twice differentiable. We also notice that
$\mathrm{dom}(-\log_{\chi}) \supseteq \mathbb{R}_+$.
To show the equivalence, we extract $\chi$ from any
twice differentiable $f$-divergence and show that for this couple $(f,
\chi)$,
$KL_{\chi}(P\|Q) = I_f(P\|Q), \forall P, Q$. Let $f_\diamond(z)
\defeq z \cdot f(1/z)$ denote the Csisz\'ar dual of $f$, which is
also convex (indeed, $f''_\diamond(z) = (1/z^2)\cdot f''(z)$) and
satisfies $I_f(P\|Q) = I_{f_\diamond}(Q\|P)$. Hence, we want to prove
\begin{eqnarray}
\expect_{\X\sim P}\left[-\log_{\chi}\left(\frac{Q(\X)}{P(\X)}\right)\right] & = & \expect_{\X\sim P}
\left[f_\diamond \left(\frac{Q(\X)}{P(\X)}\right)\right]\:\:, \forall
P, Q\:\:.
\end{eqnarray}
We want 
\begin{eqnarray}
\frac{\chi'}{\chi^2} & = & f''_\diamond\:\:,
\end{eqnarray}
whose solution is easily found to be solution to the following
differential equation: $\mathrm{d}\left(-1/\chi(z)\right) = f''_\diamond(z)
\mathrm{d} z$, that is, $-1/\chi(z) = f'_\diamond(z) + k$ for any constant $k$
and therefore
\begin{eqnarray}
\chi(z) & = & -\frac{1}{f'_\diamond(z) + k}\:\:,\label{eqchif}
\end{eqnarray}
Clearly, $\chi$ is increasing since $f_\diamond$ is convex and
\begin{eqnarray}
\chi'(z) & = & \frac{f''_\diamond(z)}{(f'_\diamond(z) + k)^2}\:\:.
\end{eqnarray}
 We now
constrain the choice of $k$ to the fact that we also want $\chi(z)\geq
0$, that is, we want $k$ such that 
\begin{eqnarray}
f'_\diamond(z) & \leq & -k\:\:, \forall z\in \mathbb{R}_+\:\:.\label{constK}
\end{eqnarray}
To prove that this is indeed possible, we first remark
that for any constant $k_2\geq 0$, 
\begin{eqnarray}
f'(t) & \leq & f'(t) + t f''(t) + k_2 \:\:,\forall t\geq 0\:\:.\label{eqCONV1}
\end{eqnarray}
This is indeed obvious since $f$ is convex, and it brings after
integration between any constant $c \in \mathrm{dom} f'$ and $z$,
$f(z) - f(c) \leq z f'(z) - c f'(c) + k_2 (z-c)$, which
brings after the change of variable $z\mapsto 1/z$ and reordering:
\begin{eqnarray}
\underbrace{f\left(\frac{1}{z}\right) - \frac{1}{z} \cdot
f'\left(\frac{1}{z}\right)}_{= f'_\diamond(z)} & \leq & \frac{k_2}{z} + f(c) - cf'(c) - ck_2 \:\:,
\end{eqnarray}
so we get that we can pick $k_2=0$ which, to guarantee ineq. (\ref{constK}), yields \textit{e.g.} the choice
\begin{eqnarray}
k & = & -(f(c) - cf'(c)) = - f'_\diamond(1/c)\:\:, \label{eqKA}
\end{eqnarray}
with $c \in \mathrm{dom} f'$. For the
expression of $\chi$ in (\ref{eqchif}), we obtain 
\begin{eqnarray}
-\log_{\chi}(z) & = & \int_1^{z} (f'_\diamond(t) + k)\mathrm{d}t \nonumber\\
 & = & f_\diamond(z) - f_\diamond(1) + k (z-1)\:\:.
\end{eqnarray}
So,
\begin{eqnarray}
KL_{\chi}(P\|Q) & \defeq & \expect_{\X\sim
  P}\left[-\log_{\chi}\left(\frac{Q(\X)}{P(\X)}\right)\right]
\nonumber\\
 & = & \expect_{\X\sim
  P}\left[f_\diamond \left(\frac{Q(\X)}{P(\X)}\right)\right] - \expect_{\X\sim
  P}\left[f_\diamond(1) \right] + k \cdot \expect_{\X\sim
  Q}\left[1 \right] - k \cdot \expect_{\X\sim
  P}\left[1 \right]
\nonumber\\
 & = & \expect_{\X\sim
  P}\left[f_\diamond \left(\frac{Q(\X)}{P(\X)}\right)\right] - f_\diamond(1) + k - k 
\nonumber\\
 & = & \expect_{\X\sim
  P}\left[f_\diamond
  \left(\frac{Q(\X)}{P(\X)}\right)\right] \label{eq000}\\
 & = & I_{f_\diamond}(Q\|P) \nonumber\\
 & = & I_f(P\|Q) \:\:,
\end{eqnarray}
as claimed. Eq. (\ref{eq000}) comes from the fact that $f_\diamond(1)
= f(1) = 0$ by assumption. Remark to finish that fixing $k$ as in
eq. (\ref{eqKA}) yields
\begin{eqnarray}
-\log_{\chi}(z) & = & f_\diamond(z) - f_\diamond(1) - (z-1)
f'_\diamond\left(\frac{1}{c}\right)\label{eqLOG1}\:\:.
\end{eqnarray}
If we fix $c = 1$, which is guaranteed to be in $\mathrm{dom} f$, then
we obtain the expression of a Bregman divergence:
\begin{eqnarray}
-\log_{\chi}(z)  & = & D_{f_\diamond}(z\|1)\label{eqLOGCHI1}\:\:.
\end{eqnarray}
In this case, from
eq. (\ref{eqchif}) and our choice of $c$ (and therefore $k$),
\begin{eqnarray}
\chi(z) & = & -\frac{1}{f'_\diamond(z) - f'_\diamond(1)}\nonumber\\
 & = & -\frac{1}{\frac{\mathrm{d} D_{f_\diamond}(z\|1)}{\mathrm{d}z}}\:\:.\label{eqchif2}
\end{eqnarray}
Otherwise, it is possible to tune $c$ in eq. (\ref{eqchif}) or directly
$k$ in ineq. (\ref{constK})
to achieve
additional constraints while keeping the non-negativity of
$\chi$.\\

\noindent We prove point (ii). We have
\begin{eqnarray*}
\expect_{\tilde{{Q}}}[-(\log_\chi({P})-\log_\chi({Q}))]
& = &
\expect_{\tilde{{Q}}}[-(\log_\chi({P})-\log_\chi(\tilde{{Q}}))]
+ \expect_{\tilde{{Q}}}[-(\log_\chi(\tilde{{Q}})-\log_\chi({Q}))]\:\:.
\end{eqnarray*}
Also, 
\begin{eqnarray}
(\log_\chi({P})-\log_\chi({\tilde{{Q}}})) & = & \int_{{{1}}}^P
\frac{1}{\chi(t)} \cdot \mathrm{d}t - \int_1^{\tilde{{Q}}}
\frac{1}{\chi(t)} \cdot \mathrm{d}t\nonumber\\
& = & \int_{\tilde{{Q}}}^P
\frac{1}{\chi(t)} \cdot \mathrm{d}t\nonumber\\
 & = & \int_{1}^{\frac{P}{\tilde{{Q}}}}
\frac{\tilde{{Q}}}{\chi(t \tilde{{Q}})} \cdot \mathrm{d}t\nonumber\\
 & = & \int_{1}^{\frac{P}{\tilde{{Q}}}}
\frac{1}{\chi_{\tilde{{Q}}}(t)} \cdot \mathrm{d}t\nonumber\\
 & = & \log_{\chi_{\tilde{{Q}}}}\left(\frac{P}{\tilde{{Q}}}\right)\:\:,
\end{eqnarray}
with 
\begin{eqnarray}
\chi_{\tilde{{Q}}(\ve{x})}(t) & \defeq & \frac{1}{\tilde{{Q}} (\ve{x})}\cdot \chi
(t\tilde{{Q}}(\ve{x}))\label{defCHITILDE} 
\end{eqnarray}
satisfying $\mathrm{d} \chi_{\tilde{{Q}} (\ve{x})} /
\mathrm{d} t = \chi'
(t \tilde{{Q}} (\ve{x}))$ and so is increasing, plus $\chi_{\tilde{{Q}}}$ is
positive iff $\chi$ is positive since $\tilde{{Q}}(\ve{x})\geq 0$, so $\chi_{\tilde{{Q}}}(t)$
defines a
$\chi$-logarithm, also differentiable. Hence,
\begin{eqnarray}
\expect_{\tilde{{Q}}}[-(\log_\chi({P})-\log_\chi(\tilde{{Q}}))] & = & KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|P)\:\:,
\end{eqnarray}
and
\begin{eqnarray}
\expect_{\tilde{{Q}}}[-(\log_\chi({Q}) - \log_\chi(\tilde{{Q}}))] & = & KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|Q)\:\:.
\end{eqnarray}
This ends the proof of point (ii).\\

\noindent We prove point (iii). Since $-\log_{\chi}$ is convex, it
follows from Legendre duality,
\begin{eqnarray}
KL_{\chi_{\tilde{{Q}}}}(\tilde{Q}\|P) & = & \sup_{T:
  \mathcal{X}\rightarrow \mathbb{R}} \left\{\expect_{P} [T(\ve{x})]  -
\expect_{\tilde{Q}}
[(-\log_{\chi_{\tilde{Q}}})^\star(T(\ve{x}))]\right\}\nonumber\\
 & = & \sup_{T:
  \mathcal{X}\rightarrow \mathbb{R}} \left\{\expect_{P} [T(\ve{x})]  -
\expect_{\tilde{Q}}
[(-\log_{\chi_{\tilde{Q}}})^\star(T(\ve{x}))]\right\}\nonumber\\
 & = & \sup_{T:
  \mathcal{X}\rightarrow \mathbb{R}} \left\{\expect_{P} [T(\ve{x})]  -
\expect_{\tilde{Q}}
[\log_{\chi^{\bullet}_{\tilde{Q}}} (T(\ve{x}))]\right\} \:\:, \label{varprob}
\end{eqnarray}
with 
\begin{eqnarray}
\chi^{\bullet}(z) & \defeq & \frac{1}{\chi^{-1}\left(\frac{1}{-z}\right)}\:\:.
\end{eqnarray}
The last eq. comes from the following. $-\log_{\chi}$ being
differentiable, its Legendre conjugate has derivative the inverse of the
derivative of $-\log_{\chi}$. Since $(-\log_{\chi})'(z) = -1/\chi(z)$,
its inverse is found to be $((-\log_{\chi})')^{-1}(z) =
\chi^{-1}(-1/z)$, which therefore corresponds to a
$\chi^\bullet$-logarithm with $\chi^\bullet(z) = 1/\chi^{-1}(-1/z)$,
as claimed. Notice that
\begin{eqnarray}
(\log_{\chi^{\bullet}})''(z)  = (1/\chi^\bullet)'(z) & = & \frac{1}{z^2} \cdot \frac{1}{\chi'\left(\chi^{-1}\left(\frac{1}{-z}\right)\right)}\:\:,
\end{eqnarray}
which is non-negative and proves the \textit{convexity} of
$\log_{\chi^{\bullet}}$. To finish-up the proof of point (iii), we
show that the optimal solution $T^*(\ve{x})$ to the variational problem in
eq.(\ref{varprob}) is indeed $T^*(\ve{x}) = -\tilde{Q}(\ve{x}) /
\tilde{P}(\ve{x})$. A pointwise differentiation of eq. (\ref{varprob})
yields that at the optimum, we have 
\begin{eqnarray}
P(\ve{x}) - \tilde{Q}(\ve{x})\cdot \left(
\log_{\chi^\bullet_{\tilde{Q}}}\right)'(T(\ve{x}))) & = & 0\:\:,
\end{eqnarray}
that is, exploiting the fact that $\chi^\bullet(z) = 1/\chi^{-1}(-1/z)$,
\begin{eqnarray}
T^*(\ve{x}) & = & \left(\left(
\log_{\chi^\bullet_{\tilde{Q}}}\right)'\right)^{-1}\left(\frac{P(\ve{x})}{\tilde{Q}(\ve{x})}\right) \nonumber\\
 & = & \left(\frac{1}{\chi^\bullet_{\tilde{Q}}}\right)^{-1}\left(\frac{P(\ve{x})}{\tilde{Q}(\ve{x})}\right) \nonumber\\
 & = &
 -\frac{1}{\chi_{\tilde{Q}} \left(\frac{P(\ve{x})}{\tilde{Q}(\ve{x})}\right)} \label{eqCHIBULLET}\\
 & = &
 -\frac{\tilde{Q}(\ve{x})}{\chi
   \left(\frac{P(\ve{x})}{\tilde{Q}(\ve{x})} \cdot \tilde{Q}(\ve{x})\right)}\nonumber\\
 & = &
 -\frac{\tilde{Q}(\ve{x})}{\chi
   (P(\ve{x}))}\nonumber\\
 & = & - \frac{\tilde{Q}(\ve{x})}{\tilde{P}(\ve{x})}\:\:.\label{eqCHIBUL2}
\end{eqnarray}
In eq. (\ref{eqCHIBULLET}), we have used the fact that
$(1/\chi^\bullet)^{-1}(z) = - 1/\chi(z)$. Notice that because of the
normalization of the escorts, the optimal $T^*$ simplifies to
\begin{eqnarray}
T^*(\ve{x}) & = & - \frac{\chi(Q(\ve{x}))}{\chi(P(\ve{x}))}\:\:.
\end{eqnarray}

